Measuring dependencies between variables of a dynamical system using fuzzy affiliations

A statistical, data-driven method is presented that quantifies influences between variables of a dynamical system. The method is based on finding a suitable representation of points by fuzzy affiliations with respect to landmark points using the Scalable Probabilistic Approximation algorithm. This is followed by the construction of a linear mapping between these affiliations for different variables and forward in time. This linear mapping can be directly interpreted in light of unidirectional dependencies and relevant properties of it are quantified. These quantifications then serve as measures for the influences between variables of the dynamics. The validity of the method is demonstrated with theoretical results and on several numerical examples, including real-world basketball player movement.

==> basketballResults.tex <==
\subsection{Full basketball dependency results}
\label{sec:basketballresults}
Order of players in all rows and columns: (Dallas) Williams, Matthews, Parsons, Nowitzki, Pachulia, (Cleveland) Irving, Smith, James, Love, Thompson.\\
Dependencies from one player to himself are omitted, therefore the zeros are placed on the diagonals.


\textbf{Dallas attacking}
\begin{equation*}
M_{\Vert \cdot \Vert_1} = \begin{pmatrix} 
0&2.31&2.47&1.76&1.7&2.94&2.29&2.27&1.83&1.9\\\ 
2.3&0&2.09&1.71&2.05&1.9&2.78&2.07&2.04&1.55\\\ 
2.63&2.35&0&1.76&2&2.23&2.52&2.77&1.85&2.13\\\ 
2.05&1.96&1.79&0&1.76&2.05&2.02&1.99&2.17&1.94\\\ 
2.14&2.49&2.2&1.57&0&2.27&2.47&2.2&2.18&2.08\\\ 
2.84&1.92&2.33&1.51&1.82&0&2.25&2.23&1.96&1.99\\\ 
2.13&2.48&2.22&1.66&1.88&2.08&0&2.39&2.29&1.75\\\ 
2.42&1.99&2.71&1.58&1.8&2.55&2.02&0&2.13&1.87\\\ 
2.1&2.32&1.97&2.03&2.07&2.37&2.72&2.09&0&1.73\\\ 
2.31&1.77&2.59&1.85&1.96&2.52&2.22&2.38&1.78&0\\\ 
\end{pmatrix}
\end{equation*}


\begin{equation*}
   M_{\nu} = 0.01\cdot
\begin{pmatrix} 
0&1.51&1.71&0.52&0.49&2.73&1.15&1.1&0.48&0.75\\\ 
1.37&0&0.87&0.53&1.24&0.56&2.49&1.04&0.86&0.27\\\ 
1.89&1.43&0&0.66&0.86&1.25&1.83&2.45&0.57&1.21\\\ 
0.89&0.79&0.41&0&0.57&1.35&0.83&1.01&1.29&0.97\\\ 
1.13&1.74&1.1&0.27&0&1.2&1.77&1.21&1.09&1.02\\\ 
2.42&0.6&1.41&0.24&0.54&0&1.08&1.23&0.69&0.76\\\ 
0.96&1.5&1.21&0.34&0.68&0.85&0&1.57&1.27&0.62\\\ 
1.51&0.74&2.22&0.29&0.52&1.67&0.84&0&1.38&0.57\\\ 
0.83&1.37&0.79&0.96&0.92&1.38&2.55&1.06&0&0.56\\\ 
1.41&0.51&1.92&0.68&0.81&1.95&1.13&1.69&0.49&0\\\ 
\end{pmatrix}
\end{equation*}

\textbf{Cleveland attacking}
\begin{equation*}
M_{\Vert \cdot \Vert_1} = 
\begin{pmatrix} 
0&2.04&2.71&1.99&1.78&2.89&2.19&2.11&1.62&1.62\\\ 
2.05&0&2.26&2.22&1.9&2.28&2.54&1.81&1.64&1.82\\\ 
2.49&2.22&0&2.08&1.77&2.21&2.1&2.53&1.89&1.96\\\ 
2.01&2.5&1.89&0&1.97&2.51&1.81&1.97&2.49&1.99\\\ 
2.04&2.42&2&2&0&1.9&1.95&1.84&1.72&2.02\\\ 
2.89&2.25&2.01&2.37&1.66&0&2.41&2.52&2.08&1.75\\\ 
1.97&2.46&2.07&1.76&1.6&1.96&0&2.14&2.03&1.82\\\ 
2.11&1.66&2.27&1.91&1.65&2.26&2.01&0&1.89&1.78\\\ 
1.79&1.99&1.99&2.09&1.57&1.88&2.34&2.1&0&1.63\\\ 
2.13&2.4&2.33&2.26&2.11&2.23&2.33&2.29&1.86&0\\\ 
\end{pmatrix}
\end{equation*}

\begin{equation*}
M_{\nu} = 0.01\cdot
\begin{pmatrix} 
0&0.97&2.27&0.93&0.66&2.71&1.04&1.13&0.33&0.31\\\ 
0.83&0&1.21&1.13&0.89&1.28&2.13&0.64&0.31&0.61\\\ 
1.58&1.24&0&1.14&0.58&1.29&0.86&1.83&0.61&0.74\\\ 
0.7&1.45&0.49&0&0.75&1.93&0.51&0.76&1.79&0.75\\\ 
0.85&1.54&0.83&0.66&0&0.65&0.73&0.53&0.39&0.91\\\ 
2.48&1.05&0.9&1.53&0.35&0&1.81&1.81&0.95&0.45\\\ 
0.67&1.8&0.84&0.43&0.33&0.71&0&1.11&0.85&0.64\\\ 
1.16&0.29&1.29&0.81&0.38&1.28&0.66&0&0.57&0.6\\\ 
0.63&0.79&0.74&1.02&0.24&0.58&1.42&1.01&0&0.39\\\ 
1.01&1.56&1.2&1.49&1.04&1.31&1.19&1.57&0.78&0\\\ 
\end{pmatrix}
\end{equation*}
